Risk-Controlling Model Selection via Guided Bayesian Optimization

Adjustable hyperparameters of machine learning models typically impact various key trade-offs such as accuracy, fairness, robustness, or inference cost. Our goal in this paper is to find a configuration that adheres to user-specified limits on certain risks while being useful with respect to other conflicting metrics. We solve this by combining Bayesian Optimization (BO) with rigorous risk-controlling procedures, where our core idea is to steer BO towards an efficient testing strategy. Our BO method identifies a set of Pareto optimal configurations residing in a designated region of interest. The resulting candidates are statistically verified and the best-performing configuration is selected with guaranteed risk levels. We demonstrate the effectiveness of our approach on a range of tasks with multiple desiderata, including low error rates, equitable predictions, handling spurious correlations, managing rate and distortion in generative models, and reducing computational costs.

==> sections_rev/acknowledgments.tex <==
\section*{Acknowledgments}
We thank the anonymous reviewers and members of the  Barzilay and  Jaakkola research groups for helpful discussions and feedback.
B.L.G. is supported in part by the CHE Data Science fellowship, the Zuckerman-CHE STEM Leadership Program, the Schmidt Futures Israeli Women’s Postdoctoral Award and the Technion Viterbi Fellowship. 
A.F. is supported in part by the NSF Graduate
Research Fellowship. This work is also supported in part by
the ML for Pharmaceutical
Discovery and Synthesis (MLPDS) Consortium and the DARPA Accelerated Molecular Discovery program.

==> sections_rev/pruning.tex <==
\section{Multi-dimensional pruning}
\label{sec:pruning_details}
First, we describe the core model units and introduce some essential notation, while keeping the exact model implementation as general as possible. Second, we describe each of the pruning dimensions, its associated importance score, and the thresholding mechanism.

\subsection{Transformer model}
Consider a Transformer model~\citep{vaswani2017attention,devlin2018bert} with $K$ layers. The input to the model is given as a sequence of $L$ (for notational simplicity we omit here the dependency of the length on $x$) tokens $x=\left(x_1,\ldots,x_{L}\right)$, which are first mapped to learneable word embeddings $e=\left(e_1,\ldots,e_L\right)$. Tokens are then passed through the model's layers, with $h_j=\left(h_{j,1},\ldots,h_{j,L}\right)$ denoting the $j$-th layer hidden representation. Each layer consists of a multi-head attention, with $W$ heads producing the combined output $a_j = \sum_{w=1}^W\textrm{Attn}_{j,w}(h_{j-1})$, which is followed by a feed-forward network to provide the next layer hidden representation. The last layer is attached to a classification head with $|\mathcal{Y}|$ outputs, where $f(x,y)$ denotes the output of class $y$. The model is optimized by minimizing a loss function $\mathcal{L}$ computed empirically over the training set. 

\subsection{Token pruning}
It is often the case that the input consists of a large amount of tokens that have a negligible contribution for the prediction task. The idea in token pruning is to identify unimportant tokens and discard them at some point in the model.   

To identify the contribution of each token, we attach to each layer a token importance predictor $s^\textrm{tok}_j: \mathcal{X}\rightarrow \mathbb{R}$ based on the token hidden representation $h_{j,l}$. Following~\citep{modarressi2022adapler}, we use as importance scores gradient attributions, computed by:
\begin{equation}
    r_l= \left\|\frac{\partial f(x,y_c)}{\partial e_l}\odot e_l\right\|_2
\end{equation}
where $y_c$ is the true label, and $\odot$ denotes element-wise product. The token importance predictors in each layer are optimized with a cross-entropy loss, where the labels are the scores, normalised to sum to one. In the $j$-th layer, tokens with $s^\textrm{tok}_j(x_l)<\lambda^\textrm{tok}$ are pruned and are not transferred to next layer. The number of tokens remaining after pruning is given by $L_j(x;\lambda^\textrm{tok})=\sum_{l=1}^L\bigcap_{j'=1}^j\mathbf{1}\left\{s^\textrm{tok}_{j'}(x_l)>\lambda^\textrm{tok}\right\}$.

\subsection{Early exiting}
Early-exiting is based on the idea that examples vary in their difficulty level, hence, require different amount of computation to reach to a good prediction. While for simple examples a decision can be made early on, difficult examples may require going through the full model.  
We attach a prediction head $f_j: \mathcal{X}\rightarrow \mathcal{Y}$ to each layer, trained to predict the labels via the same loss function as the original model. Following~\cite{liu2020fastbert}, we define the importance score based on the prediction head entropy:
\begin{equation}
    s^\textrm{layer}_j(x)=\sum_{y \in |\mathcal{Y}|} p_j(y|x)\log p_j(y|x)  
\end{equation}
where $p_j(y|x)$ are the per-class probabilities provided by the $j$-th prediction head. Based on this score, examples with $s^\textrm{layer}_j(x) < \lambda^\textrm{layer}$ exit in the $j$-th layer. The exit layer of $x$ is given by $K_\textrm{exit}(x;\lambda^\textrm{layer})=\argmin_j \left\{j\in\{1,\ldots,K\} \Big| s^\textrm{layer}_j(x) < \lambda^\textrm{layer}\right\}$. 

\subsection{Head pruning}
It was shown by \citet{michel2019sixteen} that a significant fraction of attention heads can be removed with a little impact on the performance.  
Each attention head $(w,j), \> 1\leq j \leq K, 1\leq w \leq W$ is assigned a score $s^\textrm{head}_j(w)$ according to:
\begin{equation}
    s^\textrm{head}_j(w) = \left |\textrm{Attn}_{j,w}(h_{j-1})^T\frac{\partial \mathcal{L}}{\partial\textrm{Attn}_{j,w}(h_{j-1})}\right  |.
\end{equation}
The scores in each layer are normalized to sum to one.
Attention heads with $s^\textrm{head}_j(w)<\lambda^\textrm{head}$ are pruned. The number of heads left after pruning is given by $W_j(\lambda^\textrm{head})=\sum_{w=1}^W\mathbf{1}\left\{s^\textrm{head}_j(w)>\lambda^\textrm{head}\right\}$. Note that this is a fixed pruning, unlike the previous pruning dimensions that vary according to the input $x$. 
